Robust Reinforcement Learning Objectives for Sequential Recommender Systems

Attention-based sequential recommendation methods have shown promise in accurately capturing users' evolving interests from their past interactions. Recent research has also explored the integration of reinforcement learning (RL) into these models, in addition to generating superior user representations. By framing sequential recommendation as an RL problem with reward signals, we can develop recommender systems that incorporate direct user feedback in the form of rewards, enhancing personalization for users. Nonetheless, employing RL algorithms presents challenges, including off-policy training, expansive combinatorial action spaces, and the scarcity of datasets with sufficient reward signals. Contemporary approaches have attempted to combine RL and sequential modeling, incorporating contrastive-based objectives and negative sampling strategies for training the RL component. In this work, we further emphasize the efficacy of contrastive-based objectives paired with augmentation to address datasets with extended horizons. Additionally, we recognize the potential instability issues that may arise during the application of negative sampling. These challenges primarily stem from the data imbalance prevalent in real-world datasets, which is a common issue in offline RL contexts. Furthermore, we introduce an enhanced methodology aimed at providing a more effective solution to these challenges. Experimental results across several real datasets show our method with increased robustness and state-of-the-art performance.

==> sections/appendices.tex <==
\newpage
\appendix

==> sections/background.tex <==

\section{Problem Statement}
The goal is to learn a policy from offline data that, when applied online, optimizes total rewards from user interactions. This is achieved through a framework integrating sequential modeling and reinforcement learning, capturing user behavior patterns. Sequential models predict future user actions based on historical data and have proven effective in recommender systems, outperforming traditional collaborative filtering methods due to their ability to capture temporal dynamics and user-item interactions.

\subsection{Self-Attentive Sequential Recommendation}
The SASRec method \citep{SASRec}, a self-attentive sequential recommendation model, uses the Transformer architecture for next-item predictions in recommender systems. It emphasizes understanding intricate temporal patterns and dependencies in user-item interactions, offering a detailed insight into user preferences.
The Transformer model uses its self-attention function to assign weights to different items in the user's history, effectively identifying the items most relevant to the user's current situation. By analyzing  the user's interaction sequence, it formulates a context-aware representation of the user's behavior. This assists in predicting the subsequent item in the sequence, yielding personalized, context-sensitive recommendations. SASRec's application of the Transformer model evidences its efficacy in addressing shifting user preferences, resulting in superior recommendations and enhanced user satisfaction.



==> sections/introduction_2.tex <==
\section{Introduction}
Recommender systems (RS) are the requisite component of many modern product offerings. By allowing personalized content and product recommendations, such systems power applications ranging from e-commerce, social media, entertainment and news. The realization of this importance was the impetus behind much active research in the past decade, driven by the increasing need to model user behavior and preferences over time. Traditional collaborative filtering techniques, which rely on user-item interaction history, have been widely adopted to predict user preferences. However, these methods often fail to capture the complex temporal dynamics and contextual information that govern user behavior. Sequential models appeared as an alternative model family, more closely dedicated to modeling the context and order of user-item interactions.

RNNs were an early solution to the importance of sequential modelling, as demonstrated by \citep{wu2017recurrent, yu2016dynamic}. Uni-directional architectures were later superseded by bidirectional RNNs or Transformers~\citep{NIPS2017_3f5ee243}: such models are better able to capture the subtleties of user behavior sequences, since they don't adhere to a strict order like language or time-series data. Such developments are however limited by the fact that sequence modelling is only a part of the overall problem: high-performing recommender systems also require accounting for changing dynamics, the tradeoff between long- and short- term gain, and finally balancing the tradeoff between exploration and exploitation in the space of potential user actions. All of these concerns are better addressed by ~\emph{learning a policy}, i.e. by incorporating reinforment learning (RL) into the training pipeline. Reinforcement learning offers an appealing framework for this purpose, as it enables the recommender system to learn an optimal policy through interaction with the environment, balancing the trade-off between exploration and exploitation. By incorporating RL into the recommendation process, the system can actively adapt to changing user preferences and item catalogs, maximizing long-term user satisfaction rather than merely focusing on immediate rewards.




Recommender systems (RS) have become an indispensable tool for providing personalized content and product recommendations to users across various domains, such as e-commerce, social media, entertainment, and news. 
In the past decade, there have been significant advancements in the field of sequential recommendation, driven by the increasing need to model user behavior and preferences over time. Traditional collaborative filtering techniques, which rely on user-item interaction history, have been widely adopted to predict user preferences. However, these methods often fail to capture the complex temporal dynamics and contextual information that govern user behavior. To address these limitations, sequential models have emerged as a promising alternative, enabling the modeling of user preferences in a more context-aware manner by considering the order of user-item interactions.
Advances in sequential modeling have been significantly enhanced by powerful RNN-based models, as demonstrated by \citep{wu2017recurrent, yu2016dynamic}. Unidirectional RNNs process input sequences from left to right, which might not always optimally capture the subtleties of user behavior sequences, since they don't adhere to a strict order like language or time-series data.
Using bidirectional models like RNNs and Transformers \citep{NIPS2017_3f5ee243} in user behavior sequences aids in a deeper understanding of user preferences, improving recommendation accuracy by capturing dependencies in both directions.  
In addition to improving the modeling of user-item interactions, it is crucial to optimize the recommendation strategy itself. Reinforcement learning (RL) offers an appealing framework for this purpose, as it enables the recommender system to learn an optimal policy through interaction with the environment, balancing the trade-off between exploration and exploitation. By incorporating RL into the recommendation process, the system can actively adapt to changing user preferences and item catalogs, maximizing long-term user satisfaction rather than merely focusing on immediate rewards.

\begin{figure}[t]
    \centering
    %\captionsetup{justification=left}
    \includegraphics[width=135mm]{Figures/architecture/architecture.png}
    \caption{Model architecture for the training process and the interaction between the transformer model and Q-learning with the proposed objectives. CQL objective considers positive samples (green) and hard negative action sampling (red) and contrastive objective is applied batch-wise across different user items (green vs orange).}
    \label{fig:architecture}
\end{figure}

Despite the impressive achievements of language models like GPT-4 \citep{openai2023gpt4}, particularly in tasks such as next-item prediction, there still exists a wide range of challenges to be addressed. Additional research is imperative to formulate novel solutions to the cold-start problem, a typical scenario when data for new users or items is limited. The crux of the issue is to devise strategies that can efficiently utilize contextual information for recommendation generation in such scenarios. In addition, the design of more robust reinforcement learning mechanisms is crucial for the creation of dynamic, interactive recommender systems capable of maximizing long-term user engagement.

In this paper, we propose a novel approach for recommender systems that combines the expressive power of sequential models, particularly the Transformer architecture, with the dynamic learning capabilities of RL. \lili{Relate this part to Figure 1, also mention the stability? And also CQL?} Our method aims to capture the rich temporal context of user-item interactions while proactively guiding the learning process to optimize the recommendation strategy. Our comprehensive experimentation across multiple datasets demonstrates our method not only enhance the precision of recommendations in comparison to the baseline, but also adds further stability to the training process. Additionally, we underscore the efficacy of the RL component \lili{Maybe more details on RL component?}, highlighting its contribution to the overall system performance. Furthermore, we discuss the challenges and opportunities associated with integrating sequential models and RL within recommender systems, offering valuable insights and directions for forthcoming research in this field.

  



Our core contributions are as follows:

\begin{itemize}
    \item We investigate the application of a contrastive learning objective, in conjunction with sequential augmentation strategies, and provide empirical evidence of its effectiveness on a variety of challenging real-world datasets.
    \item We pinpoint fundamental problems arising from the inclusion of negative action sampling, as proposed in previous studies, and propose a more conservative objective to alleviate these instabilities during RL training.
    \item Our analysis underscores the need to monitor training progress for RL-based models to detect instabilities that could impair model performance in online deployment. We advocate for the reporting of training dynamics alongside tabular results in reinforcement learning and provide empirical backings for these findings. Our code is publicly available in \url{https://github.com/melfm/sasrec-ccql}.
\end{itemize}

==> sections/related_work_All.tex <==

\section{Related Work}
Our research intersects with several lines of work. In this section we will discuss the strategies and modelling frameworks that are most similar to our approach.

\subsection{Collaborative Filtering Methods}

\textbf{Matrix Factorization Extensions:}
Early works in sequential recommendation extended traditional collaborative filtering methods, such as matrix factorization, to incorporate temporal dynamics. These extensions include time-aware matrix factorization and time-decaying models, which capture the evolution of user preferences and item attributes over time. \cite{RendleFactoredMC} introduced first-order MC to capture short-term user preferences combined with matrix factorization (MF) \cite{5197422} to model long-term preferences. MF methods seek to uncover latent dimensions to represent users’ preferences and items’ properties, and estimate interactions through the inner product between the user and item embeddings \cite{Koren:2011dz}. 

\subsection{Sequential Recommendation Models:}
\mel{This is template add related work}


• SASRec [14]: This baseline is based on self-attention and
uses the Transformer [35] architecture. The output of the
Transformer encoder is treated as the latent sequence state.

\textbf{Session-based Recommendations}: With the growing importance of session data in online services, session-based recommendation methods have emerged to model short-term user preferences. These techniques focus on predicting the next item in a user's session based on their recent interactions, using methods like nearest-neighbor approaches or session-aware matrix factorization.

\textbf{Markov Chain Models}: To capture the sequential nature of user interactions, Markov chain models have been utilized for next-item prediction. These methods model the transition probabilities between items and estimate the likelihood of a user's next interaction based on their previous interactions.

\textbf{Recurrent Neural Networks (RNNs)}: RNNs, especially Long Short-Term Memory (LSTM) networks and Gated Recurrent Units (GRUs), have been widely used for sequential recommendation due to their ability to model temporal dependencies in user-item interactions. These deep learning models can capture complex user behavior patterns and generate more accurate recommendations.

\textbf{Attention Mechanisms}: Attention mechanisms, such as the self-attention used in Transformers, have been incorporated into sequential recommendation models to better capture the dependencies between user-item interactions. These models can dynamically weigh the importance of different interactions, leading to more accurate and context-aware recommendations.

\textbf{Pre-trained Language Models}: With the success of large pre-trained language models like BERT, GPT, and their variants, researchers have started to explore their applicability in sequential recommendation tasks. These models can capture complex patterns in user-item interaction sequences and generate high-quality recommendations. BERT4Rec \citep{sun2019bert4rec} applies the BERT model to sequential recommendation tasks, capturing sequential and contextual details from users' past interactions with items. This results in more accurate, personalized recommendations. 

\subsection{Reinforcement Learning Approaches:}
There has been growing interest in applying reinforcement learning to sequential recommendation, with techniques like Q-learning, Deep Q-Networks (DQNs), and policy gradient methods being utilized. RL-based models can optimize long-term user satisfaction and adapt to changing user preferences over time

\textbf{Model-based RL} approaches \cite{chen2019generative, NEURIPS2019_e49eb652} attempt
to eliminate the off-policy issue by building a model to simulate the environment. The policy can then be trained through interactions
with the simulator. Two-stage approaches depend heavily on the accuracy of the simulator. Although related methods, such as generative adversarial networks (GANs) \cite{NIPS2014_5ca3e9b1}, achieve good performance when generating content like images and speeches, simulating users’ responses is a much more complex and difficult task.

\textbf{Contrastive Learning}
Contrastive Learning for Sequential
Recommendation (CL4SRec) \cite{CL4SRec}
builds on top of SASRec with an added constrastive learning objective. However this work does not consider RL component and therefore is demonstrated on static recommendation datasets without rewards. In this work, we consider this as a baseline for SASRec with a contrastive objective.

\textbf{Deep RL for recommendation}  Several work has attempted utilizing RL for recommendation.
\cite{XiangyuNegativePairwise} proposed to utilize negative sampling along with Q-learning. \cite{RewShapingRecommend2022} build their method on top of the REINFORCE algorithm. Let the policy $\pi$ assume a functional form, mapping states to actions, parameterized by $\theta \in \mathbf{R}^d$. However their framework operates in an \textit{offline} RL setting, adopting importance weighting in batch offline RL, applying top-$K$ off-policy correction scheme.

Recently with Transformer's success in NLP tasks, these transformer based models are introduced to sequential recommendation \citep{SASRecAC, SASRecSA2C, sun2019bert4rec}. SASRec in \cite{SASRecAC, SASRecSA2C} uses a two-layer Transformer decoder to capture user’s sequential behaviors. SASRec is a unidirectional model using a casual attention mask. 

Bandit algorithms that also rely on reward signal and reward expectation maximization have also been investigated. Bandits however assume taking actions does not affect the state as they model a one-state MDP. Since recommendations have affect on user behavior, RL is a more suitable framework.

\mel{TODO Read and Cite Bo's paper - Relates to stabalizing RL for rec }
\cite{tang2023improving}


\subsection{Graph-based Methods:}
GNNs have been employed to model the complex relationships between users and items in a graph-based representation. By capturing higher-order connectivity patterns, GNNs can generate more accurate and context-aware sequential recommendations.

==> tabulat_results.tex <==
\begin{center}
\small % Change font size to small
\setlength{\tabcolsep}{4pt} % Adjust column spacing

% Center the caption and add it on top of the table
\captionsetup{justification=centering} % Center the caption
\captionof{table}{Top-$k$ recommendation performance comparison of different models ($k$ = 5, 10, 20) on RSC \textcolor{red}{I think this is the same as RC15 (RecSys15 YooChoose) ?}.}
\label{table:rsccomp}

\begin{adjustbox}{max width=\linewidth} % Scale the table to fit the linewidth
\begin{tabular}{l c *{6}{c} *{6}{c}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Reward@20} & \multicolumn{6}{c}{Purchase} & \multicolumn{6}{c}{Click} \\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
 &  & HR@5 & NG@5 & HR@10 & NG@10 & HR@20 & NG@20 & HR@5 & NG@5 & HR@10 & NG@10 & HR@20 & NG@20 \\
\midrule
NextItNet & 360 & 0.209 & 0.150 & 0.290 & 0.177 & 0.385 & 0.201 & 0.302 & 0.231 & 0.387 & 0.259 & 0.460 & 0.277 \\
NextItNet-AC & 348 & 0.243 & 0.180 & 0.291 & 0.195 & 0.361 & 0.213 & 0.348 & 0.268 & 0.400 & 0.285 & 0.463 & 0.300 \\
Caser & 287 & 0.200 & 0.146 & 0.262 & 0.166 & 0.317 & 0.180 & 0.229 & 0.171 & 0.285 & 0.190 & 0.335 & 0.203 \\
GRU & 442 & 0.259 & 0.178 & 0.378 & 0.217 & 0.435 & 0.231 & 0.422 & 0.314 & 0.528 & 0.349 & 0.614 & 0.370 \\
GRU-AC & 264 & 0.182 & 0.109 & 0.248 & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
SASRec & 464 & 0.278 & 0.196 & 0.397 & 0.234 & 0.481 & 0.256 & 0.427 & 0.304 & 0.521 & 0.334 & 0.594 & 0.353 \\
SASRec-AC & 458 & 0.332 & 0.231 & 0.399 & 0.253 & 0.475 & 0.273 & 0.442 & 0.316 & 0.528 & 0.343 & 0.605 & 0.363 \\
\textbf{SASRec-CO} & 485 & 0.308 & 0.220 & 0.404 & 0.251 & 0.483 & 0.270 & 0.421 & 0.304 & 0.525 & 0.338 &  0.592 & 0.355 \\
SNQN & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
CL4Rec & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}



\begin{center}
\small % Change font size to small
\setlength{\tabcolsep}{4pt} % Adjust column spacing

% Center the caption and add it on top of the table
\captionsetup{justification=centering} % Center the caption
\captionof{table}{Top-$k$ recommendation performance comparison of different models ($k$ = 5, 10, 20) on Taobao.}
\label{table:taobtao}

\begin{adjustbox}{max width=\linewidth} % Scale the table to fit the linewidth
\begin{tabular}{l c *{6}{c} *{6}{c}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Reward@20} & \multicolumn{6}{c}{Purchase} & \multicolumn{6}{c}{Click} \\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
 &  & HR@5 & NG@5 & HR@10 & NG@10 & HR@20 & NG@20 & HR@5 & NG@5 & HR@10 & NG@10 & HR@20 & NG@20 \\
\midrule
NextItNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
MF & 152 & 0.089 & 0.072 & 0.101 & 0.076 & 0.119 & 0.080 & 0.113 & 0.082 & 0.131 & 0.087 & 0.156 & 0.094 \\
\textcolor{red}{MF-AC} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
SASRec & 112 & 0.064 & 0.047 & 0.071 & 0.050 & 0.090 & 0.054 & 0.077 & 0.057 & 0.095 & 0.063 & 0.114 & 0.067 \\
\textbf{SASRec-CO} & 126 & 0.042 & 0.033 & 0.052 & 0.036 & 0.067 & 0.040 & 0.121 & 0.096 & 0.141 & 0.102 & 0.164 & 0.108 \\
SNQN & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
CL4Rec & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\textcolor{red}{SA2C} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
